Regularizing Deep Networks by Modeling and Predicting Label Structure

We construct custom regularization functions for use in supervised training of deep neural networks. Our technique is applicable when the ground-truth labels themselves exhibit internal structure; we derive a regularizer by learning an autoencoder over the set of annotations. Training thereby becomes a two-phase procedure. The first phase models labels with an autoencoder. The second phase trains the actual network of interest by attaching an auxiliary branch that must predict output via a hidden layer of the autoencoder. After training, we discard this auxiliary branch. We experiment in the context of semantic segmentation, demonstrating this regularization strategy leads to consistent accuracy boosts over baselines, both when training from scratch, or in combination with ImageNet pretraining. Gains are also consistent over different choices of convolutional network architecture. As our regularizer is discarded after training, our method has zero cost at test time; the performance improvements are essentially free. We are simply able to learn better network weights by building an abstract model of the label space, and then training the network to understand this abstraction alongside the original task.

==> Makefile <==
# programs
PDFLATEX = pdflatex
CP       = cp
RM       = rm
GREP     = grep
DIFF     = diff -q
TOUCH    = touch

# input and output files
TEXFILE = label-reg_arxiv.tex
PDFFILE = label-reg_arxiv.pdf
TEXINCLUDES = $(wildcard include/*)

# intermediate files
TEXLOG     = $(basename $(TEXFILE)).log
AUXFILE    = $(basename $(TEXFILE)).aux
OLDAUXFILE = $(AUXFILE).old

# arxiv submission files
ARXIV_FILES := $(if $(wildcard files.txt),$(shell cat files.txt),)
ARXIV_OUT   := arxiv.tar.gz

# If this message appears in TEXLOG, we must re-run LaTeX.
RERUNLATEX = "Rerun to get cross-references right"

# The primary target (created by the command "make") is the PDF file.
.PHONY: pdf
pdf: $(PDFFILE)

# This rule uses PDFLaTeX to create a PDF file from a LaTeX file.
# Then PDFLaTeX is re-run to resolve references, as necessary.
$(PDFFILE): $(TEXFILE) $(TEXINCLUDES)
	$(TOUCH) $(AUXFILE)
	$(CP) $(AUXFILE) $(OLDAUXFILE)
	$(PDFLATEX) $<
	while $(GREP) -q $(RERUNLATEX) $(TEXLOG); do $(PDFLATEX) $<; done

# arxiv submission
.PHONY: submit
submit: $(ARXIV_OUT)
$(ARXIV_OUT): files.txt $(ARXIV_FILES)
	@COPYFILE_DISABLE=1 tar cvzfh $(ARXIV_OUT) $(ARXIV_FILES)

# This rule cleans out the files made by the make process.
clean:
	$(RM) -f $(AUXFILE)\
                 $(OLDAUXFILE)\
                 $(TEXLOG)\
                 $(PDFFILE)\
                 $(ARXIV_OUT)

